Sur la torsion de Frobenius de la cat\'egorie des modules instables

In the category $\mathcal{P}_{d}$ of strict polynomial functors, the morphisms between extension groups induced by the Frobenius twist are injective. In \cite{Cuo14a}, the category $\mathcal{P}_{d}$ is proved to be a full sub-category of the category $\mathcal{U}$ of unstable modules \textit{via} Hai's functor. The Frobenius twist is extended to the category $\mathcal{U}$ but remains mysterious there. This article aims to study the Frobenius twist and its effects on the extension groups of unstable modules. We compute explicitly several extension groups and show that in these cases, the morphisms induced by the Frobenius twist are injective. These results are obtained by constructing the minimal injective resolution of the free unstable module $F(1)$.

==> morphismes.tex <==
\definecolor{qqqqff}{rgb}{0,0,1}
\definecolor{cqcqcq}{rgb}{0.75,0.75,0.75}
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=2.8cm,y=1.4cm]
\draw [color=cqcqcq,dash pattern=on 1pt off 1pt, xstep=1.4cm,ystep=0.7cm] (-0.5,-0.5) grid (3.5,6.75);
\draw[->,color=black] (-0.5,0) -- (3.5,0);
\foreach \x in {1}
\draw[shift={(\x,0)},color=black] (0pt,2pt) -- (0pt,-2pt) node[below] {\footnotesize $I_{(\x)}$};
\foreach \x in {2}
\draw[shift={(\x,0)},color=black] (0pt,2pt) -- (0pt,-2pt) node[below] {\footnotesize $I_{(\x)}$};
\draw[->,color=black] (0,-0.5) -- (0,6.5);
\foreach \x in {3}
\draw[shift={(\x,0)},color=black] (0pt,2pt) -- (0pt,-2pt) node[below] {\footnotesize $I_{(1)}\oplus I_{(\x,1)}$};
\draw[->,color=black] (0,-0.5) -- (0,6.5);
\foreach \y in {1,2,3,4,5,6}
\draw[shift={(0,\y)},color=black] (2pt,0pt) -- (-2pt,0pt) node[left] {\footnotesize $\y$};
\draw[color=black] (0pt,-10pt) node[right] {\footnotesize };
\clip(-0.5,-0.5) rectangle (3.5,6.75);
\draw [-] (1,3) -- (2,2.77);
\draw [-] (1,5) -- (2,4.77);
\draw [-] (2,2) -- (3,2);
\draw [-] (2,3.23) -- (3,3);
\draw [-] (2,4) -- (3,4);
\draw [-] (2,5.23) -- (3,5);
\draw [-] (1,1) -- (2,0);
\draw [-] (1,2) -- (2,0);
\draw [-] (1,4) -- (2,0);
\draw [-] (2,2.8) -- (3,0);
\draw [-] (1,6) -- (2,5.7);
\draw [-] (2,6.3) -- (3,6);
\begin{scriptsize}
\node[rounded corners,fill=gray!15] (S1) at (1,1) [draw] {$u$};
\node[rounded corners,fill=white] (S2) at (1,2) [draw] {$u^2$};
\node[rounded corners,fill=white] (S0) at (1,0) [draw] {$0$};
\node[rounded corners,fill=gray!15] (S3) at (1,3) [draw] {$u^3$};
\node[rounded corners,fill=white] (S4) at (1,4) [draw] {$u^4$};
\node[rounded corners,fill=gray!15] (S5) at (1,5) [draw] {$u^5$};
\node[rounded corners,fill=white] (S6) at (1,6) [draw] {$u^6$};

\node[rounded corners,fill=gray!15] (Si) at (3,1) [draw] {$u$};
\node[rounded corners,fill=white] (Si) at (3,2) [draw] {$u^2$};
\node[rounded corners,fill=white] (Si4) at (3,0) [draw] {$0$};
\node[rounded corners,fill=gray!15] (Si) at (3,3) [draw] {$u^3$};
\node[rounded corners,fill=white] (Si) at (3,4) [draw] {$u^4$};
\node[rounded corners,fill=gray!15] (Si) at (3,5) [draw] {$u^5$};
\node[rounded corners,fill=gray!15] (Si) at (3,4.6) [draw] {$r_{2^k+2}$};
\node[rounded corners,fill=white] (Si5) at (3,6) [draw] {$u^6$};
\node[rounded corners,fill=white] (Si) at (3,5.6) [draw] {$Sq^1r_{2^k+2}$};

\node[rounded corners,fill=white] (Si) at (2,0) [draw] {$0$};
\node[rounded corners,fill=white] (Si1) at (2,2) [draw] {$\omega_2$};
\node[rounded corners,fill=gray!15] (Si2) at (2,2.77) [draw] {$\omega_3$};
\node[rounded corners,fill=gray!15] (Si) at (2,3.23) [draw] {$\alpha$};
\node[rounded corners,fill=white] (Si) at (2,4) [draw] {$\omega_2^2$};
\node[rounded corners,fill=gray!15] (Si) at (2,5.23) [draw] {$\omega_2\alpha$};
\node[rounded corners,fill=gray!15] (Si3) at (2,4.77) [draw] {$\omega_2\omega_3$};
\node[rounded corners,fill=white] (Si51) at (2,5.6) [draw] {$\omega_3^2$};
\node[rounded corners,fill=white] (Si5) at (2,6) [draw] {$\omega_2^3$};
\node[rounded corners,fill=white] (Si6) at (2,6.4) [draw] {$\omega_3\alpha+\omega_2^3$};
\draw [-,color=qqqqff] (Si1) edge[bend left=30] node [pos=0.5,fill=gray!20,rounded corners] {$Sq^1$} (Si2);
\draw [-,color=qqqqff] (Si2) edge[bend left=50] node [pos=0.3,fill=gray!20,rounded corners] {$Sq^2$} (Si3);
\draw [-] (Si3) edge[bend left=10]  (Si4);
\draw [-,color=qqqqff] (S1) edge[bend left=30] node [pos=0.5,fill=gray!20,rounded corners] {$Sq^1$} (S2);
\draw [-,color=qqqqff] (S2) edge[bend left=50] node [pos=0.3,fill=gray!20,rounded corners] {$Sq^2$} (S4);
\draw [-,color=qqqqff] (S3) edge[bend left=50] node [pos=0.7,fill=gray!20,rounded corners] {$Sq^2$} (S5);
\draw [-,color=qqqqff] (S5) edge[bend left=30] node [pos=0.5,fill=gray!20,rounded corners] {$Sq^1$} (S6);
%\draw [-] (Si51) edge[bend left=10] (Si4);
\end{scriptsize}
\end{tikzpicture}

==> s2.tex <==
\begin{center}
\definecolor{xdxdff}{rgb}{0.49,0.49,1}
\definecolor{qqqqff}{rgb}{0,0,1}
\definecolor{cqcqcq}{rgb}{0.75,0.75,0.75}
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1.2cm,y=0.9cm]
\draw [color=cqcqcq,dash pattern=on 1pt off 1pt, xstep=1.2cm,ystep=0.9cm] (0,0) grid (8.5,8);
\draw[->,color=black] (-0.5,0) -- (8.5,0);
\foreach \x in {1}
\draw[shift={(\x,0)},color=black] (0pt,2pt) -- (0pt,-2pt) node[below] {\footnotesize $R^0$};
\foreach \x in {2}
\draw[shift={(\x,0)},color=black] (0pt,2pt) -- (0pt,-2pt) node[below] {\footnotesize $R^1$};
\foreach \x in {3}
\draw[shift={(\x,0)},color=black] (0pt,2pt) -- (0pt,-2pt) node[below] {\footnotesize $R^2$};
\foreach \x in {6}
\draw[shift={(\x,0)},color=black] (0pt,2pt) -- (0pt,-2pt) node[below] {\footnotesize
$R^{2^{n}-4}$};
\foreach \x in {7}
\draw[shift={(\x,0)},color=black] (0pt,2pt) -- (0pt,-2pt) node[below] {\footnotesize
$R^{2^{n}-3}$};
\foreach \x in {8}
\draw[shift={(\x,0)},color=black] (0pt,2pt) -- (0pt,-2pt) node[below] {\footnotesize
$R^{2^{n}-2}$};
\draw[->,color=black] (0,-1) -- (0,8);
\foreach \y in {5}
\draw[shift={(0,\y)},color=black] (2pt,0pt) -- (-2pt,0pt) node[left] {\footnotesize $2^{n}-3$};
\foreach \y in {6}
\draw[shift={(0,\y)},color=black] (2pt,0pt) -- (-2pt,0pt) node[left] {\footnotesize $2^{n}-2$};
\foreach \y in {7}
\draw[shift={(0,\y)},color=black] (2pt,0pt) -- (-2pt,0pt) node[left] {\footnotesize $2^{n}-1$};
\foreach \y in {2,3}
\draw[shift={(0,\y-1)},color=black] (2pt,0pt) -- (-2pt,0pt) node[left] {\footnotesize $\y$};

\clip(-0.45,-0.8) rectangle (8.5,8);

\draw [->] (1,7) -- (2,7);
\draw [->] (2,6) -- (3,6);
\draw [->] (6,2) -- (7,2);
\draw [-] (7,1) -- (8,1);
\draw [dash pattern=on 1pt off 1pt] (3,5)-- (6,3);
\draw [dash pattern=on 1pt off 1pt] (1,7)-- (1,0);
\draw [dash pattern=on 1pt off 1pt] (2,6)-- (2,0);
\draw [dash pattern=on 1pt off 1pt] (3,5)-- (3,0);
\draw [dash pattern=on 1pt off 1pt] (6,2)-- (6,0);
\draw [dash pattern=on 1pt off 1pt] (7,1)-- (7,0);
\draw [dash pattern=on 1pt off 1pt] (8,1)-- (8,0);
\draw [dash pattern=on 1pt off 1pt] (1,7)-- (0,7);
\draw [dash pattern=on 1pt off 1pt] (2,6)-- (0,6);
\draw [dash pattern=on 1pt off 1pt] (3,5)-- (0,5);
\draw [dash pattern=on 1pt off 1pt] (6,2)-- (0,2);
\draw [dash pattern=on 1pt off 1pt] (7,1)-- (0,1);
\begin{scriptsize}
\draw [-,color=qqqqff] (2,6) edge[bend left=40] (2,7);
\draw [-,color=qqqqff] (3,5) edge[bend left=40] (3,6);
\draw [-,color=qqqqff] (6,2) edge[bend left=40] (6,3);
\draw [-,color=qqqqff] (7,1) edge[bend left=40] (7,2);
\draw[color=qqqqff] (1.6,6.5) node {$Sq^1$};
\draw[color=qqqqff] (2.6,5.5) node {$Sq^1$};
\draw[color=qqqqff] (5.6,2.5) node {$Sq^1$};
\draw[color=qqqqff] (6.6,1.5) node {$Sq^1$};
\node[rounded corners,fill=gray!25] (y) at (1,7) [draw] {$u^{2^{n}-1}$};
\node[rounded corners,fill=gray!25] (t1) at (2,6) [draw] {$x_{2^{n}-4}$};
\node[rounded corners,fill=gray!25] (t3) at (3,5) [draw] {$x_{2^{n}-5}$};
\node[rounded corners,fill=gray!25] (t5) at (6,2) [draw] {$x_{1}$};
\node[rounded corners,fill=gray!25] (t7) at (7,1) [draw] {$x_{0}$};
\node[rounded corners,fill=gray!25] (t8) at (8,1) [draw] {$u^{2}$};
\draw[color=black] (1.6,7.4) node {$\partial_{r}^{0}$};
\draw[color=black] (2.5,6.4) node {$\partial_{r}^{1}$};
\draw[color=black] (6.5,2.4) node {$\partial_{r}^{2^{n}-4}$};
\draw[color=black] (7.5,1.4) node {$\partial_{r}^{2^{n}-3}$};
\fill [color=qqqqff] (2,7) circle (1.5pt);
\fill [color=qqqqff] (3,6) circle (1.5pt);
\fill [color=qqqqff] (6,3) circle (1.5pt);
\fill [color=qqqqff] (7,2) circle (1.5pt);
\end{scriptsize}
\end{tikzpicture}
\end{center}
